Robust Clock Skew and Offset Estimation for IEEE 1588 in the Presence of Unexpected Deterministic Path Delay Asymmetries

IEEE 1588, built on the classical two-way message exchange scheme, is a popular clock synchronization protocol for packet-switched networks. Due to the presence of random queuing delays in a packet-switched network, the joint recovery of the clock skew and offset from the timestamps of the exchanged synchronization packets can be treated as a statistical estimation problem. In this paper, we address the problem of clock skew and offset estimation for IEEE 1588 in the presence of possible unknown asymmetries between the {\color{black} deterministic path delays} of the forward master-to-slave path and reverse slave-to-master path, which can result from incorrect modeling or cyber-attacks. First, we develop lower bounds on the mean square estimation error for a clock skew and offset estimation scheme for IEEE 1588 assuming the availability of multiple master-slave communication paths and complete knowledge of the probability density functions (pdf) describing the random queuing delays. Approximating the pdf of the random queuing delays by a mixture of Gaussian random variables, we then present a robust iterative clock skew and offset estimation scheme that employs the space alternating generalized expectation-maximization (SAGE) algorithm for learning all the unknown parameters. Numerical results indicate that the developed robust scheme exhibits a mean square estimation error close to the lower bounds.

==> section5.tex <==
In this section, we present our algorithm for jointly estimating the clock skew and offset in the presence of unknown path asymmetries. As the objective function for the optimization problem in (\ref{main_equation_EM}) is not necessarily convex, proper initialization of the various parameters is necessary for the EM algorithm to ensure convergence to the global minimum instead of local minimums. We first present a simple ad-hoc scheme to obtain the initial values of the various parameters, denoted by $\hat{\bm{\Omega}}_{\pi}^{(0)}$ for the EM algorithm and then present our robust algorithm.



\subsection{Initialization for the EM algorithm}
The steps of the initialization are enumerated below:

\begin{algorithmic}[1]
	
	\STATE First, we define new variables $\gamma_i = (\phi(d_i + \tau_i) + \delta)$ and $\zeta_i = (-\phi d_i + \delta)$ for $i = 1, 2, \cdots, N$.
	

	
	\FOR {$i = 1 : N$}
	
	\STATE For a given value of $M_i$, run the EM algorithm for the GMM using the update equations given in \cite{Blimes} on  $\tilde{\bm{w}}_{1i}$ to obtain $\hat{\alpha}_{ik}^{(0)}$, $\hat{\mu}_{1ik}^{(0)}$ and $\hat{\sigma}_{1ik}^{(0)}$.
	
	\STATE For a given value of $L_i$, run the EM algorithm for the GMM using the update equations given in \cite{Blimes} on  $\tilde{\bm{w}}_{2i}$ to obtain $\hat{\beta}_{il}^{(0)}$, $\hat{\mu}_{2il}^{(0)}$ and $\hat{\sigma}_{2il}^{(0)}$.
	
	\STATE Using $\hat{\alpha}_{ik}^{(0)}$, $\hat{\mu}_{1ik}^{(0)}$ and $\hat{\sigma}_{1ik}^{(0)}$,  construct an approximate pdf of $f_{1i}(.)$, denoted by $\tilde{f}_{1i}(.)$. Similarly, using $\hat{\beta}_{il}^{(0)}$, $\hat{\mu}_{2il}^{(0)}$ and $\hat{\sigma}_{2il}^{(0)}$, construct an approximate pdf of $f_{2i}(.)$, denoted by $\tilde{f}_{2i}(.)$.
	
	\STATE Consider the timestamps $\bm{t}_{1i}$ and $\bm{t}_{2i}$ from the $i^{th}$ master-slave communication path. We have the following relationship\footnote{Since we do not have the prior information regarding on whether the $i^{th}$ path has an unknown asymmetry, we assume $\tau_i \ne 0$.}
	\begin{eqnarray}
	\bm{t}_{2i} & = & (\bm{t}_{1i} + \bm{w}_{1i})\phi + \gamma_i\bm{1}_P. \label{fwd_init_mixture} 
	\end{eqnarray}
	Relaxing the dependency constraint between $\phi$ and $\gamma_i$, we use the optimum CSOE scheme proposed in \cite{AK_Blum_offset} to obtain an estimate of $\phi$ and $\gamma_i$, denoted by $\hat{\phi}_{fwd, i}$ and $\hat{\gamma}_i$ respectively.
	
	
	\STATE Consider the timestamps $\bm{t}_{3i}$ and $\bm{t}_{4i}$ from the $i^{th}$ master-slave communication path. We have the following relationship
	\begin{eqnarray}
	\bm{t}_{3i} = (\bm{t}_{4i} - \bm{w}_{2i})\phi + \zeta_i\bm{1}_P. \label{rev_init_mixture}
	\end{eqnarray}
	Relaxing the dependency constraint between $\phi$ and $\zeta_i$, we use the optimum CSOE scheme to obtain an estimate of $\phi$ and $\zeta_i$, denoted by $\hat{\phi}_{rev, i}$ and $\hat{\zeta}_i$ respectively.
	
	\STATE We then construct the estimate of the clock skew  from the timestamps exchanged in the $i^{th}$ master-slave communication path, denoted by $\hat{\phi}_i$, as follows
	\begin{eqnarray}
	\hat{\phi}_{i} & = & (\hat{\phi}_{fwd, i} + \hat{\phi}_{rev, i})/2.
	\end{eqnarray}
	Similarly, we calculate an estimate of $\delta$, denoted by $\hat{\delta}_{i}$, from the timestamps exchanged in the $i^{th}$ master-slave communication path  as follows
	\begin{eqnarray}
	\hat{\delta}_{i} & = & (\hat{\gamma}_i + \hat{\zeta}_i)/2.
	\end{eqnarray}	


	\ENDFOR
	

	

	
	\STATE Using the obtained estimates $\hat{\phi}_i$ and $\hat{\delta}_i$ for $i = 1, 2, \cdots, N$. We fix our initial estimate of $\delta$ and $\phi$, denoted by $\hat{\delta}^{(0)}$ and $\hat{\phi}^{(0)}$, respectively, as
	\begin{eqnarray}
	\hat{\delta}^{(0)} & = & \mbox{median}\{\hat{\delta}_1, \hat{\delta}_2, \cdots, \hat{\delta}_N    \}, \\
	\hat{\phi}^{(0)} & = & \mbox{mean}\{\hat{\phi}_1, \hat{\phi}_2, \cdots, \hat{\phi}_N    \}.	
	\end{eqnarray}
	
	
	\FOR {$i = 1 : N$}
	
	\STATE Estimate the total fixed propagation delay in the forward path of the $i^{th}$ master-slave communication path as:
	\begin{eqnarray}
	\hat{d}_{fwd, i} & = & (\hat{\gamma}_i - \hat{\delta}^{(0)})/\hat{\phi}^{(0)}.
	\end{eqnarray}
	Similarly, estimate the total fixed propagation delay in the reverse path of the $i^{th}$ master-slave communication path as:
	\begin{eqnarray}
	\hat{d}_{rev, i} & = & (\hat{\delta}^{(0)} - \hat{\zeta}_i)/\hat{\phi}^{(0)}.
	\end{eqnarray}
	
	\STATE Set $\hat{\pi}_i^{(0)}$ as $\frac{e^{\left(|\hat{d}_{fwd, i} - \hat{d}_{rev, i}| - d_{\tau}\right)\kappa}}{e^{\left(|\hat{d}_{fwd, i} - \hat{d}_{rev, i}| - d_{\tau}\right)\kappa} + 1}$, where $\kappa$ is a normalization constant\footnote{We choose this value as  fixed to $10^6$ since propagation delays in the considered scenario are in the order of $\mu s$ for the considered LTE backhaul network scenario.}.
	
	
		
	\IF {$\left|\hat{d}_{fwd, i} - \hat{d}_{rev, i}\right| \le d_\tau$}
	\STATE Set $\hat{d}_i^{(0)}$ to to $(\hat{d}_{fwd, i} + \hat{d}_{rev, i})/2$.
	\STATE Set $\hat{\tau}_i^{(0)}$ to $0$.
	\ELSE
	\STATE Set $\hat{d}_i^{(0)}$ to to $\hat{d}_{rev, i}$.
	\STATE Set $\hat{\tau}_i^{(0)}$ to $(\hat{d}_{fwd, i} - \hat{d}_{rev, i})$.
	\ENDIF
	\ENDFOR
\end{algorithmic}

 
 
 \subsection{Final Algorithm}\label{EMAlgo}\label{sub2_sec5}
 %\begin{algorithm}
 %\caption{Proposed robust POE scheme}
The steps of the proposed robust clock skew and offset estimation scheme are presented in Algorithm \ref{Alg1}.
 \begin{algorithm}
 \caption{Calculate a robust estimate of $\phi$ and $\delta$}\label{Alg1}
 {
 	%	\setstretch {1.5}
 	\algsetup{indent = 2 em}
 	\begin{algorithmic}[1]
 		\STATE Initialize the parameter vector $\bm{\Omega}_{\pi}$ as $\hat{\bm{\Omega}}_{\pi}^{(0)}$.
 		\STATE Calculate the current log likelihood, denoted by $\mbox{LLF}_{cur}$, using (\ref{Incomplete_logLL}) and  $\hat{\bm{\Omega}}_{\pi}^{(0)}$. 
 		\STATE Initialize the previous value of the log likelihood $\mbox{LLF}_{prev} = -\infty$ and fix a threshold value $\epsilon$ to determine when to stop.
 		\WHILE {$\left|\mbox{LLF}_{pres} - \mbox{LLF}_{prev}\right| \ge \epsilon$}
 		\FOR {$i = 1 : N; k = 1 : M; l = 1 : M; j = 1 : P$}
 		\STATE compute $\chi_{ijkl}^{(1)}$ and $\chi_{ijkl}^{(0)}$ using (\ref{a1_ijkl}) based on current estimate $\hat{\bm{\Omega}}_{\pi}^{(m)}$.
 		\ENDFOR
 		\FOR {$i = 1 : N$}
 		\STATE update the current estimate of ${\pi}_i$ using (\ref{pi_update}).
 		\ENDFOR
 		\FOR {$i = 1 : N, k = 1 : M$}
 		%	\FOR {$k = 1 : M_i$}
 		\STATE update the current estimate of ${\alpha}_{ik}$ using (\ref{alpha_update}).
 		%	\ENDFOR
 		\ENDFOR
 		\FOR {$i = 1 : N, l = 1 : M$}
 		%	\FOR {$l = 1 : L_i$}
 		\STATE update the current estimate of ${\beta}_{il}$ using (\ref{beta_update}).
 		%	\ENDFOR
 		\ENDFOR
 		\STATE Update the current estimate of ${\bm{\Psi}}$ by solving (\ref{Remain_update}).
 		\STATE Set $\mbox{LLF}_{prev} \leftarrow \mbox{LLF}_{cur}$.
 		\STATE Update the log likelihood $\mbox{LLF}_{pres}$ using (\ref{Incomplete_logLL}) and the updated current parameter values $\hat{\bm{\Omega}}_{\pi}^{(m+1)}$.
 		\ENDWHILE
		
%		\STATE Let $\hat{\bm{\Omega}}_{\pi}$ denote the estimate of the parameters from the EM algorithm. Use $\hat{\bm{\alpha}}_i$ and $\hat{\bm{\beta}}_i$ to obtain an estimate of $\bm{a}_i$ and $\bm{b}_i$, respectively, for  $i = 1, 2, \cdots, N$.
		
		
%		\STATE Obtain an estimate of $\bm{a}_i$ using $\hat{\bm{\alpha}}_i$ for $i = 1, 2, \cdots, N$. 
%		
%		\STATE Obtain an estimate of $\bm{b}_i$ using $\hat{\bm{\beta}}_i$ for $i = 1, 2, \cdots, N$.
		
		\STATE Using the rounding method described in Section IV.B, construct the set of possible solutions of $\bm{\eta}$ by $\{ \tilde{\bm{\eta}} \}$.
		
		\STATE Using the estimates of $\hat{\bm{\alpha}}$ and $\hat{\bm{\beta}}$ obtained from the EM algorithm, solve (\ref{main_equation_CVTR}) to obtain an estimate of $\delta$ and $\phi$.

 \end{algorithmic}}
 \end{algorithm}
 %In summary, we use the EM algorithm for identifying the master-slave communication paths which have been subject to delay attacks, and employ the optimal vector location parameter estimator to estimate the phase offset of the slave node.
 

